Weighting vectors for machine learning: numerical harmonic analysis applied to boundary detection

Metric space magnitude, an active field of research in algebraic topology, is a scalar quantity that summarizes the effective number of distinct points that live in a general metric space. The {\em weighting vector} is a closely-related concept that captures, in a nontrivial way, much of the underlying geometry of the original metric space. Recent work has demonstrated that when the metric space is Euclidean, the weighting vector serves as an effective tool for boundary detection. We recast this result and show the weighting vector may be viewed as a solution to a kernelized SVM. As one consequence, we apply this new insight to the task of outlier detection, and we demonstrate performance that is competitive or exceeds performance of state-of-the-art techniques on benchmark data sets. Under mild assumptions, we show the weighting vector, which has computational cost of matrix inversion, can be efficiently approximated in linear time. We show how nearest neighbor methods can approximate solutions to the minimization problems defined by SVMs.

==> checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} In Section \ref{sec:limitations}.
  \item Did you discuss any potential negative societal impacts of your work? In Section \ref{sec:limitations}.
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} Theorem \ref{thm:w_kd_error_bound} states all assumptions and the definition used is stated in Definition \ref{def:scattered}.
	\item Did you include complete proofs of all theoretical results?
    \answerYes{} In the supplementary materials.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} In the supplementary materials.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} Section \ref{sec:outlier_detection} gives these details.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{} We can provide this if needed.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{} We did not use special compute resources.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} The reference to the data set repository \cite{Rayana:2016} appears in the caption to Table \ref{tab:outlier} in Section \ref{sec:outlier_detection}.
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> discussion.tex <==
\section{Discussion}

One limitation of the proposed method is that it suffers from the curse of dimensionality--it generally perform better when the data is not high dimensional. And although the authors do not see potential negative societal impacts of the specific work presented in this paper; they do acknowledge the potential for harm when any form of automation is taken without proper foresight and caution.

==> limitations.tex <==
\section{Limitations and discussion} \label{sec:limitations}

One limitation of the proposed method is that it suffers from the curse of dimensionality--it generally perform better when the data is not high dimensional. Another is that the theoretical guarantees for these methods hold when the data is densely and uniformly sampled from a reasonable, compact subset of $\R^n$. However, in practice we have seen that in many cases when this assumption is violated, the methods still perform reasonably well. And although the authors do not see potential negative societal impacts of the specific work presented in this paper; they do acknowledge the potential for harm when any form of automation is taken without proper foresight and caution.

==> outline.tex <==
\section*{Outline}
FIXME: REMOVE ME!

{\bf Limit is 9 pages}, not including references or paper checklist. Appendix and/or supplementary material must be separate file.
\begin{enumerate}
    \item abstract {\bf (Everybody)}
    \item intro {\bf (Everybody)}
    \item boundary detection
        \begin{enumerate}
            %\item discuss weight defined using L1 norm as a boundary detector. {\bf (Jeff) }
            \item discuss weight using L2 norm as a boundary detector. {\bf (Jeff){\color{red} If space permits, I suggest using content from Appendix B }}
            \item application to interpret bert {\bf (Dan, Suhaas)}
        \end{enumerate}
    \item connection to generalized SVMs. These things follow immediately {\bf (Jeff){\color{red} Done}}
        \begin{enumerate}
            \item classification algorithm {\bf (Jeff)}
            \item outlier detection algorithm {\bf (Jeff)}
        \end{enumerate}
    Discuss here also the pushback against the notion that it is very desirable to have a smooth kernel. {\bf (Eric, Glenn)}
    \item approximation by nearest neighbors
        \begin{enumerate}
            \item reciprocal of row sums approximates w {\bf (Eric)}
        \end{enumerate}
    \item weighting layer 
        \begin{enumerate}
            \item define weighting layer {\bf (Dan, Eric)}
        \end{enumerate}
    \item Experiments
        \begin{itemize}
            \item outlier detection {\bf (Jeff){\color{red}Done}}
            \item outlier detection with DNN+Mag layer?
            \item DNN+Mag layer basic classification results {\bf (Dan, Eric)}
            \item approximation of $w$ using  {\bf (Eric)}
                \begin{itemize}
                    \item $1/f$
                    \item nearest neighbors (approx of $1/f$)
                \end{itemize}
        \end{itemize}
    \item Conclusions {\bf (Everybody)}
\end{enumerate}

==> related_work.tex <==
\section{Related work} \label{sec:related_work}

==> weighting_layer.tex <==
\section{Weighting layer}\label{sec:weighting_layer}

In this section we define a neural network layer, denoted ${\bf Weight}$, inspired by the weighting vector. We provide example architectures using this layer, along with appropriate loss functions. This layer computes the weighting vector of a collection of \emph{anchor points}, with learnable coordinates, with respect to a randomly initialized target vector, and treats each training batch as a kernelized SVM prediction.

\begin{definition}
Define the \emph{weighting layer} as 

\begin{equation}
    {\bf Weight}_{(A, y_A)}(X) = \z_{AX}^Tw_A
\end{equation}

where $X$ is an $b \times d$ matrix, where $b$ denotes the batch size, and $d$ is the feature vector dimension. $A$ is a $k \times d$ matrix, where $k$ is a chosen number of points with learnable coordinates, referred to as \emph{anchor points}, and $y_A$ is a length $k$ column vector with entries randomly initialized from a uniform distribution supported on the range of the output specific to the task at hand (e.g. between 0 and number of classes for classification). The vector $w_A$ is the solution to $\z_Aw = y_A$, and $\z_{AX}$ is the $k \times b$ whose $(i, j)$ entry is $\exp{(-t\norm{a_i - x_j}_2)}$, where $t$ is learned on a per-batch basis from the batch inputs. When context is clear, we will simply write ${\bf Weight}$ without reference to the anchor points.
\end{definition}

We have seen in Section \ref{sec:boundarydetect} that one of the constraints for which the weighting is an effective boundary detector is that the data points should be densely, uniformly sampled from a reasonable region in $\R^d$. While arbitrary data sets may not have this property, preceding layers to ${\bf Weight}$ may act as transformations taking the original data set to densely, uniformly sampled regions. 

In practice, we have observed the following general architecture to be successful when employing a weighting layer. First, fully connected layers with softsign activation. Then a {\bf Weight} layer; and finally, fully connected layers that are appropriate for the learning task at hand. Empirically, we have found that the loss function of the form

\begin{equation}
    L(X, y) = L_{pred}(X, y) + \norm{\z_{AX}^Tw_A - y_A}_1
\end{equation}

performs well, where $L_{pred}$ is the prediction loss appropriate to the task. The term $\norm{\z_{AX}^Tw_A - y_A}_1$ can be seen by using Eqn. \ref{eqn:disjoint_gluing_Ybar} (Appdx. \ref{sec:appendix}) to be minimizing the weight of the points of X, thereby maximizing the weight of the anchor points.
